Handle decomposition complexity and representation spaces

We prove that there are homology three-spheres that bound definite four-manifolds, but any such bounding four-manifold must be built out of many handles. The argument uses the homology cobordism invariant $\Gamma$ from instanton Floer homology.

==> complex-Yn.tex <==
%!TEX root = Gamma-PHS.tex


\section{Filtered $\mathcal{SO}$-complexes and instanton homology}

{\color{red} The definition of filtered $\mathcal{SO}$-complexes will be given in this section and the construction of $\widetilde C_*(Y)$ will be sketched here.}

\section{Flat Connections on $Y_n$}

For an integer homology sphere $Y$, the Floer complex $C_*(Y)$ is generated by the non-trivial critical points of the Chern-Simons functional, perhaps after a perturbation. The critical points of the Chern-Simons functional are in correspondence  with the isomorphism classes of flat $\SU(2)$-connections on $Y$, or equivalently the conjugacy class of space of representations of the fundamental group of $Y$ into $\SU(2)$. It is easy to characterize the space of isomorphism classes of flat $\SU(2)$-connections on $Y_n$, which we denote by $\chi_n$. The space $\chi_n$ always contains the trivial connection, and we denote the complement of this element by $\chi_n^*$. The space $\chi_1$ consists of three elements, the trivial connection $\Theta$ and two irreducible flat connections $\alpha$, $\beta$. 
More generally, we have:
\[
  \chi_{n+1}^*=\chi_1^*\times \chi_{n}^*\times \SO(3)\sqcup \chi_1^*\sqcup \chi_{n}^*
\]
The first term in the above expression is obtained by gluing irreducible flat connections on $Y_{n}$ and $Y_1$ where there is an $\SO(3)$ gluing factor. The second term is the result of gluing an irreducible flat connection on $Y_1$ to the trivial connection on $Y_{n}$. Finally the last term is given similarly where the role of $Y_1$ and $Y_{n}$ is reversed.

%The chain group $C_*(Y_1)$ is freely generated by the elements of $\chi_1$. However, the connected sum theorem that we used in the previous section does not necessarily guarantee that the chain group $C_*(Y_n)$, that we used for higher values of $n$, is generated by critical points of the Chern-Simons functional or even a perturbation of it. It only asserts that $C_*(Y_n)$ together with the differential $d_n$ provide the same information as the chain complex which is given by the critical points of (a perturbation of) the Chern-Simons functional up to chain homotopy. However, one can see relation between the algebraic complex of the previous section and the geometry of the character variety. In fact, the chain complex $C_*(Y_n)$ can be identified with the total cohomology group of $\chi_{n+1}^*$ where we use $\Lambda$ as the coefficient ring. In this section, we wish to move in this direction and obtain more information between the Floer homological data of the previous section and the space $\chi_n$.
%
%Our starting point is that the Chern-Simons functional of $Y_n$ is Morse-Bott with the critical manifold $\chi_n$. Since the trivial connection is non-degenerate, we focus on $\chi_n^*$.
%
%
%
%Any flat connections on $Y_n=Y_1\# Y_{n-1}$ can be restricted to $Y_1$ and $Y_{n-1}$ to obtain flat connections on these manifolds. In the other direction, an irreducible flat connection on $Y_1$ can be glued to an irreducible flat connection to obtain an $\SO(3)$-worth of 
%
%
%We denote the space of flat connections on $Y_n$, up to isomorphism, by $\chi_n$. This space can be identified with the space of representations of the fundamental group of $Y_n$ into $\SU(2)$. 
%
%The chain group $C_*(Y_1)$ in the previous section is freely generated by non-trivial critical points of the Chern-Simons function of the Poincar\'e homology sphere.



